Sampling-Based Motion Planning: A Comparative Review

Sampling-based motion planning is one of the fundamental paradigms to generate robot motions, and a cornerstone of robotics research. This comparative review provides an up-to-date guideline and reference manual for the use of sampling-based motion planning algorithms. This includes a history of motion planning, an overview about the most successful planners, and a discussion on their properties. It is also shown how planners can handle special cases and how extensions of motion planning can be accommodated. To put sampling-based motion planning into a larger context, a discussion of alternative motion generation frameworks is presented which highlights their respective differences to sampling-based motion planning. Finally, a set of sampling-based motion planners are compared on 24 challenging planning problems. This evaluation gives insights into which planners perform well in which situations and where future research would be required. This comparative review thereby provides not only a useful reference manual for researchers in the field, but also a guideline for practitioners to make informed algorithmic decisions.

==> deprecated/deprecated.tex <==
\section{Comparative Evaluation: Problem Set}
\fixme{Reorganization ideas start}
We should try to reorganize the problems in a coherent order. The main points that we discussed with lydia are the following.
\begin{enumerate}
    \item We should include easy or average problems as well, where everyone is doing well to demonstrate the successes of sampling-based planners.
    \item A more (historically) coherent ordering of the problems would be the following.
    We start with easy/average problems, and move to more difficult problems such as more high-dimentional problems. Then we could include narrow passages and then we could say that if at the limit the narrrow passages become constraints, and that is where such methods are introduced such as contraints. Finally we top it off with the time-space stuff which includes dynamic obstacles. \textbf{note:} Maybe we should discuss how the perform with control problems as well. 
    \item The multirobot problems in the high-dimetional category a) and c) might be better if they are moved to a multi-robot category or are not included since the dilute a bit the core motion planning problem. Problem a) is very decentralized and can be made artificially harder by adding more and more robots. Also a decentralized planner or something like dRRT would be more appropriate here. Similarly problem c) is artificially hard since the arm does not really matter and we mostly care about the position of the bases. Problem b) is interesting since there is interplay between the three arms and could fit in this category as the last problem.      
    \item We should rethink the usage of variations in problems (and hyperplan) where things do not matter that much e.g. at free-flying robots for example, or when the environment is static.
\end{enumerate}


An Altenrative Organization:
\subsection{Standard Motion Planning Problems}
Showcase some easy problems where sampling based planners are very successful in increasing order of dimensionality:   

%https://github.com/ompl/omplapp/tree/main/resources
\begin{itemize}
    \item RandomPolygonsPlannar (2D Planning) 
    \item UniqueMazeSolving (2D Planning) 
    \item Apartment (SE(3)) Planning
    \item Home (SE(3)) Planning
    \item UR5 Table Top Planning (6D) 
\end{itemize}

Maybe we could split in two categories for real robots 

\subsection{High-Dimensional Problems}
\begin{itemize}
    \item Panda Table Top Planning (7D) 
    \item Fetch Box Planning (8D) 
    \item Baxter double arm planning (14D)
    \item Shadowhand grasping (31D) 
    \item Three-panda arms (21D)    
\end{itemize}

\subsection{Narrow Passages}
\fixme{maybe split these in the other categories}  
Narrow passages are one of the essential problem for sampling-based planning, due to the sampling measure going towards zero inside of a region which is essential for planning success. Such problems are notoriously difficult to solve. See Fig.~\ref{fig:experiments:narrowpassage}.

\begin{itemize}
    \item Bugtrap
    \item Double Bugtrap
    \item Double-Lshape
    \item Chain Egress
    \item Hypercube
    \item Fetch in deep boookshelf
    \item Shadohand in Cage 
\end{itemize}

\subsection{Manifolds}

Planning on manifolds requires that we have a way to uniformly sample and have correct interpolation and metric methods. Those experiments are a way to showcase which algorithms are applicable to general manifold spaces. We also like to showcase specific manifold (apart from euclidean space), if a specific algorithm can only solve that manifold(s). See Fig.~\ref{fig:experiments:manifold}.

\begin{itemize}
    \item Sphere
    \item Torus
    \item Klein bottle
    \item Mobius strip
    \item SE(3) or SO(3)
    \item SO(3) x SO(3) x SO(3)
\end{itemize}

\section{Comparative Evaluation: Results}

\subsection{Feasibility Problems}
\begin{itemize}
    \item Run all algorithms which try to find feasible solutions on problem set
    \item Compare according to average runtime over 10-100 runs. 
\end{itemize}

\subsection{Optimality Problems}
\begin{itemize}
    \item Run all star/optimal versions on problem set under the same cost function
    \item Plot cost/runtime to visualize which planner converges the fastest
\end{itemize}

%\input{evaluations/optimality_graphs}

%\newpage
%\subsection{Special Cases Experiments}
%
%Experiments which are special cases/ edge cases of motion planning
%
%FOR SURE:
%\begin{enumerate}
%    \item Unbounded state space: Planning in Space Time (1D space + 1D time ?). ST-RRT* only.
%
%    \item Arbitrary cost function: Maximize Clearance (2D + clearance cost function). EIT*, RRT*?
%
%    \item Infeasible planning problem (determine probabilistic infeasibility) \cite{li2021learning, li2022exponential}. Maybe use the bugtrap you already have.
%    
%    \item Non-standard manifold. Planning on KleinBottle.
%    
%\end{enumerate}
%
%MAYBE:
%\begin{itemize}
%    
%    \item Hybrid system (discrete + continuous)
%    
%    \item Hypercube (projections + highdim). QRRT*, QMP*.
%    
%    \item Non-standard goal region. Multiple goal states or IK-sampling (continuously sampled). How to deal with them: Continuously sampling.
%    \end{itemize}
%
%\newpage

%\input{images/figure_manifolds}
%\input{images/figure_narrow_passages}
%\input{images/figure_high_dimensionality}
%\input{images/figure_spacetime}
%\input{images/figure_benchmark_system}
%
%\input{experiments/figure_experiments}
%\input{images/list_of_results}
%\input{images/list_of_planner_on_experiments}


%%\begin{table}
%    \centering
%    \begin{tabular}{|c|l|}
%        \hline
%        Roadmap-based & PRM, PRM*, SPARS \\
%        Tree-based & RRT, RRT*, LBT-RRT, TRRT, EST, FMT \\
%        Informed & BIT*, InformedRRT*, AIT*, EIT*, ABIT*\\
%        Projection & KPIECE, PDST, QRRT, QMP \\
%        Kinodynamic & SST*, AO-RRT\\
%        \hline
%    \end{tabular}
%    \caption{Categories of planners.}
%\end{table}


\begin{itemize}
    \item Probabilistic Roadmap Planner (PRM)
    \item Rapidly-exploring random tree (RRT)
    \item Fast marching trees (FMT)
    \item Expansive Space trees (EST)
    \item Informed Trees
    \item KPIECE
    \item Path-Directed Subdivision Tree (PDST)
    \item SPARS
    \item LBTRRT
    \item TRRT
    \item Stable sparse trees (SST)
    \item Search Tree with Resolution Independent Density Estimation (STRIDE)
\end{itemize}


==> deprecated/deprecated_discussion.tex <==
\section{Discussion and Practical Advice}

While most motion planner are supposed to be general-purpose, i.e. solving any valid motion planning problem, it is often difficult to apply planners to a given scenario. In this section, we give helpful practical advice, which is essential in successfully running motion planning experiments.

-- PLanner selection: HOw do you choose a planner for a specific problem? Decision tree?
-- Hyperparameter tuning
--
% Planner selection (use hyperparameters to figure out which is actually better). First plan of attack is to use RRTConnect for geometric then PRM, then try other planners like BIT*., and kRRT for dynamic scenarios. 
% Scenario robustness (use variations and procedural generation to 


%% Purpose of section: Explain difficulties on making planner work on scenarios
%% - Tuning of parameters is difficult and important. How can we actually make this better?
One of the most difficult aspects of motion planning is the tuning of hyperparameters for a given scenario. This involves the extension step size in configuration space, but also the tuning of the nearest neighbor radius, or the goal bias.

- How to alleviate those difficulties:
-- Handtuning. Experience to select parameters, simple order-of-magnitude search (i.e. select one of $0.1$, $0.01$, $0.001$,...)
-- Automated tuning~\cite{cano2018automatic, moll2021hyperplan}
-- Tuning during execution based on progress (no progress -> make step size smaller. Lots of progress -> make step size larger)
-- Removing parameters. I.e. extension step size could be replaced by move-until-collision, or by using a task-space step size. Nearest neighbor radius can be chosen optimally to guarantee optimality. Goal bias 

Every planner has to be properly tested to verify its merit. However, we often see new planners being developed without having a proper set of scenarios to test them on.

- How to alleviate this
-- Procedural benchmark generation (Vary some environments, or start/goal). \cite{Chamzas2021}.
-- Select scenarios based on specific problem you want to solve (spot welding scenarios, car driving)



==> evaluations/optimality_graphs.tex <==
\begin{figure*}
    \centering
\def\width{0.32\linewidth}
\def\height{3cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth,height=\height]{evaluations/Extensions/ConstraintImplicitChain.pdf}
\caption{5D Implicit Chain}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth,height=\height]{evaluations/Extensions/ConstraintSphere.pdf}
\caption{2D constrained sphere}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth,height=\height]{evaluations/Extensions/hypercube_10.pdf}
\caption{10D Hypercube}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{Experiments \label{fig:experiments:manifold}.}

\end{figure*}

==> evaluations/table_results.tex <==
\newcolumntype{V}{>{\centering\arraybackslash}m{.033\linewidth}}
\newcolumntype{Z}{>{\raggedleft\arraybackslash}m{.01\linewidth}}
\newcolumntype{+}{!{\vrule width 1.2pt}}
\begin{table*}[t]
\centering
\renewcommand{\cellrotangle}{90}
\renewcommand\theadfont{\bfseries}
\settowidth{\rotheadsize}{\theadfont 02D Kleinbottle}
\footnotesize\centering
\renewcommand{\arraystretch}{1.2}
\setlength\tabcolsep{3pt}
\begin{tabularx}{\linewidth}{|ZX+X|X|X|X|X|X|X|}\hline
& & \multicolumn{7}{>{\centering}p{.8\textwidth}|}{List of Scenarios}\\\cline{3-9}
\multicolumn{2}{|>{\centering}p{2.5cm}+}{\rothead{Motion Planner}}
 & \rothead{02D Sphere} 
 & \rothead{02D Kleinbottle} 
 & \rothead{03D} 
 & \rothead{06} 
 & \rothead{02D Torus} 
 & \rothead{06D Apartment} 
 & \rothead{06D} 
 \\ \hline
1 & \mbox{RRTXstatic} & $0.130\color{gray}{\pm 0.035}$ & $0.144\color{gray}{\pm 0.045}$ & $-$ & $1.756\color{gray}{\pm 0.877}$ & $0.111\color{gray}{\pm 0.000}$ & $6.133\color{gray}{\pm 3.656}$ & $-$ \\ 
2 & \mbox{BiTRRT} & $\textbf{0.021}\color{gray}{\pm 0.003}$ & $0.003\color{gray}{\pm 0.001}$ & $-$ & $0.450\color{gray}{\pm 0.137}$ & $0.004\color{gray}{\pm 0.000}$ & $\textbf{0.351}\color{gray}{\pm 0.307}$ & $-$ \\ 
3 & \mbox{SBL} & $-$ & $-$ & $-$ & $4.231\color{gray}{\pm 1.023}$ & $-$ & $4.757\color{gray}{\pm 2.828}$ & $-$ \\ 
4 & \mbox{RLRT} & $0.375\color{gray}{\pm 0.087}$ & $0.061\color{gray}{\pm 0.030}$ & $-$ & $10.000\color{gray}{\pm 0.183}$ & $0.052\color{gray}{\pm 0.003}$ & $10.000\color{gray}{\pm 0.392}$ & $-$ \\ 
5 & \mbox{SORRT*} & $-$ & $-$ & $-$ & $-$ & $-$ & $10.000\color{gray}{\pm 0.044}$ & $-$ \\ 
6 & \mbox{BFMT} & $0.098\color{gray}{\pm 0.015}$ & $0.028\color{gray}{\pm 0.001}$ & $-$ & $0.910\color{gray}{\pm 0.054}$ & $0.043\color{gray}{\pm 0.000}$ & $1.374\color{gray}{\pm 0.104}$ & $-$ \\ 
7 & \mbox{RRTConnect} & $0.033\color{gray}{\pm 0.001}$ & $\textbf{0.002}\color{gray}{\pm 0.000}$ & $\textbf{0.006}\color{gray}{\pm 0.000}$ & $\textbf{0.274}\color{gray}{\pm 0.154}$ & $\textbf{0.002}\color{gray}{\pm 0.000}$ & $1.043\color{gray}{\pm 0.623}$ & $1.000\color{gray}{\pm 0.000}$ \\ 
8 & \mbox{LBTRRT} & $0.121\color{gray}{\pm 0.019}$ & $0.112\color{gray}{\pm 0.004}$ & $-$ & $1.122\color{gray}{\pm 0.111}$ & $0.111\color{gray}{\pm 0.000}$ & $5.000\color{gray}{\pm 3.844}$ & $-$ \\ 
9 & \mbox{FMT} & $0.168\color{gray}{\pm 0.030}$ & $0.058\color{gray}{\pm 0.002}$ & $-$ & $1.302\color{gray}{\pm 0.054}$ & $0.101\color{gray}{\pm 0.003}$ & $1.422\color{gray}{\pm 0.118}$ & $-$ \\ 
10 & \mbox{BKPIECE1} & $-$ & $-$ & $-$ & $1.120\color{gray}{\pm 0.438}$ & $-$ & $1.124\color{gray}{\pm 0.849}$ & $-$ \\ 
11 & \mbox{PRM} & $1.000\color{gray}{\pm 0.002}$ & $1.000\color{gray}{\pm 0.001}$ & $-$ & $10.000\color{gray}{\pm 0.021}$ & $1.000\color{gray}{\pm 0.001}$ & $10.000\color{gray}{\pm 0.028}$ & $-$ \\ 
12 & \mbox{STRIDE} & $-$ & $-$ & $-$ & $8.547\color{gray}{\pm 1.822}$ & $-$ & $3.806\color{gray}{\pm 3.595}$ & $-$ \\ 
13 & \mbox{ProjEST} & $-$ & $-$ & $-$ & $7.162\color{gray}{\pm 1.147}$ & $-$ & $4.732\color{gray}{\pm 3.604}$ & $-$ \\ 
14 & \mbox{kABIT*} & $-$ & $-$ & $-$ & $1.111\color{gray}{\pm 0.000}$ & $-$ & $1.333\color{gray}{\pm 0.471}$ & $-$ \\ 
15 & \mbox{RRT} & $0.037\color{gray}{\pm 0.006}$ & $0.008\color{gray}{\pm 0.001}$ & $-$ & $0.295\color{gray}{\pm 0.099}$ & $0.003\color{gray}{\pm 0.000}$ & $4.770\color{gray}{\pm 3.822}$ & $-$ \\ 
16 & \mbox{BiRLRT} & $0.351\color{gray}{\pm 0.193}$ & $0.002\color{gray}{\pm 0.000}$ & $-$ & $1.983\color{gray}{\pm 1.583}$ & $0.002\color{gray}{\pm 0.000}$ & $7.536\color{gray}{\pm 3.077}$ & $-$ \\ 
17 & \mbox{PRM*} & $0.297\color{gray}{\pm 0.099}$ & $0.111\color{gray}{\pm 0.000}$ & $-$ & $6.056\color{gray}{\pm 3.206}$ & $0.111\color{gray}{\pm 0.000}$ & $5.222\color{gray}{\pm 2.933}$ & $-$ \\ 
18 & \mbox{SST} & $1.000\color{gray}{\pm 0.000}$ & $0.858\color{gray}{\pm 0.108}$ & $-$ & $10.000\color{gray}{\pm 0.000}$ & $0.813\color{gray}{\pm 0.120}$ & $6.933\color{gray}{\pm 3.878}$ & $-$ \\ 
19 & \mbox{AIT*} & $-$ & $-$ & $-$ & $6.033\color{gray}{\pm 3.120}$ & $-$ & $1.633\color{gray}{\pm 0.881}$ & $-$ \\ 
20 & \mbox{EST} & $0.163\color{gray}{\pm 0.029}$ & $0.005\color{gray}{\pm 0.001}$ & $-$ & $7.459\color{gray}{\pm 1.229}$ & $0.003\color{gray}{\pm 0.000}$ & $3.060\color{gray}{\pm 3.545}$ & $-$ \\ 
21 & \mbox{kBIT*} & $-$ & $-$ & $-$ & $1.111\color{gray}{\pm 0.000}$ & $-$ & $1.200\color{gray}{\pm 0.301}$ & $-$ \\ 
22 & \mbox{InformedRRT*} & $-$ & $-$ & $-$ & $1.211\color{gray}{\pm 0.318}$ & $-$ & $6.222\color{gray}{\pm 3.932}$ & $-$ \\ 
23 & \mbox{TRRT} & $0.028\color{gray}{\pm 0.035}$ & $0.013\color{gray}{\pm 0.001}$ & $-$ & $0.608\color{gray}{\pm 0.181}$ & $0.005\color{gray}{\pm 0.000}$ & $3.006\color{gray}{\pm 3.681}$ & $-$ \\ 
24 & \mbox{RRT*} & $0.133\color{gray}{\pm 0.036}$ & $0.121\color{gray}{\pm 0.017}$ & $0.111\color{gray}{\pm 0.000}$ & $1.156\color{gray}{\pm 0.218}$ & $0.111\color{gray}{\pm 0.000}$ & $6.567\color{gray}{\pm 3.791}$ & $\textbf{1.000}\color{gray}{\pm 0.000}$ \\ 
25 & \mbox{KPIECE1} & $-$ & $-$ & $-$ & $0.774\color{gray}{\pm 0.194}$ & $-$ & $3.364\color{gray}{\pm 3.629}$ & $-$ \\ 
26 & \mbox{PDST} & $-$ & $-$ & $-$ & $1.041\color{gray}{\pm 0.670}$ & $-$ & $8.472\color{gray}{\pm 2.663}$ & $-$ \\ 
27 & \mbox{BiEST} & $0.055\color{gray}{\pm 0.019}$ & $0.003\color{gray}{\pm 0.000}$ & $-$ & $4.877\color{gray}{\pm 0.965}$ & $0.003\color{gray}{\pm 0.000}$ & $0.599\color{gray}{\pm 0.385}$ & $-$ \\ 
\hline
\end{tabularx}
\caption{Runtime (s) of 0 runs with 27 planning algorithms on 7 scenarios         with cut-off time limit of 1.00s.     Entry '$-$' means that planner does not support this planning scenario.}
\end{table*}

==> images/figure_basic_rrt.tex <==
\begin{wrapfigure}{R}{0.5\textwidth}
    \begin{minipage}{0.5\textwidth}
    \vspace*{-1.5cm}
    \begin{algorithm}[H]
    	\scriptsize
    	\caption{Basic-RRT \label{alg:rrt}}
    	\begin{algorithmic}[1]
        \Procedure{Basic-RRT}{$\xi$}  
        \State T.addNode($\xi$)
            \For{PTC is false}%$i = 1 ,\ldots, N$} 
    		\State $\x_{rand} \gets $ sample from $\X$
    		\State $\x_{near} \gets $ nearest node in T to $\x_{rand}$ 
    		\State $\x_{new} \gets$ Extend $x_{near}$ towards $x_{rand}$
    		\State $e \gets$ Local plan $x_{new}$ to $x_{near}$
    		 \If{$e \in \Xfree$}
    		\State  T.addEdge($e$) 
    		\EndIf
            \EndFor
        \State \Return T
        \EndProcedure
    \end{algorithmic}
    \end{algorithm}
    \end{minipage}
\end{wrapfigure}

==> images/figure_benchmark_system.tex <==
\begin{figure*}
    \centering
\def\width{0.48\linewidth}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/system/generation.pdf}
\caption{Generation of variations.}
\end{subfigure}\hfill
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/system/benchmark.pdf}
\caption{Evaluation pipeline (for each planner, each environment, each 100 runs).}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/system/evaluation1.pdf}
\caption{Table of Relative Improvement after hyperplan optimization.}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/system/evaluation2.pdf}
\caption{Table of absolute runtime after hyperplan optimization.}
\end{subfigure}
\caption{Evaluation methodology \label{fig:benchmark}.}
\end{figure*}

==> images/figure_high_dimensionality.tex <==
\begin{figure*}
    \centering
\def\width{0.16\linewidth}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/multirobot_24D_fixed.png}
\caption{This is multi-robot artificial, increase of the statespace. 24D three panda robots need to attain grasp position.}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/manipulation_37D_shadowhand.png}
\caption{37D ShadowHand robot grasping a ball.}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/highdimensional/fetch.png}
\caption{07D Fetch Robot, I can do them after we figure them}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/highdimensional/baxter.png}
\caption{14D Baxter}
\end{subfigure}
\caption{High-Dimensional Planning Problems \label{fig:experiments:highdimensionality}.}
\end{figure*}

==> images/figure_manifolds.tex <==
\begin{figure*}
    \centering
\def\width{0.16\linewidth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/manifold/manifold_02D_sphere.png}
\caption{2D manifold sphere}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/manifold/manifold_02D_torus.png}
\caption{2D manifold torus}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/manifold/manifold_02D_kleinbottle.png}
\caption{2D manifold Klein bottle}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/manifold/TorusMaze.png}
\caption{2D torus maze}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/manifold/SphereMaze.png}
\caption{2D sphere maze}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/manifold/ImplicitChain.png}
\caption{Implicit Chain}
\end{subfigure}
\caption{Manifold Experiments \label{fig:experiments:manifold}.}
\end{figure*}

==> images/figure_narrow_passages.tex <==
\begin{figure*}
    \centering
\def\width{0.16\linewidth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/narrowpassage/02_Disk_Opening.png}
\caption{2D Disk, which has to traverse a tight opening.}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/narrowpassage/06D_bugtrap.png}
\caption{6D Bugtrap, where a cylindrical robot needs to escape.}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/narrowpassage/06D_double_lshape.png}
\caption{6D Double L-shape, needs to traverse opening.}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{evaluations/NarrowPassages/06D_Spirelli.png}
\caption{06D Spiral}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/narrowpassage/manipulation_08D_franka.png}
\caption{8D Franka Emica Panda arm navigating into a box.}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/narrowpassage/10D_Chain_Twister.png}
\caption{10D Kinematic chain, needs to traverse twister.}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{Narrow Passage Experiments \label{fig:experiments:narrowpassage}.}
\end{figure*}

==> images/figure_scenarios.tex <==
\begin{table}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
        \includegraphics[width=\linewidth]{evaluations/Classical/06D_Apartment.png}

    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> images/figure_spacetime.tex <==
\begin{figure*}
    \centering
\def\width{0.16\linewidth}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/spacetime/narrow_scenario.pdf}
\caption{Planning for a 2D disk robot in narrow passage.}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/spacetime/rnd.png}
\caption{Planning for a 8D disk robot to navigate between several randomly, but known, moving disks.}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/spacetime/mobilemanip.png}
\caption{Planning for one 8D mobile manipulator with space-time constraints.}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/spacetime/fixedmanip.png}
\caption{7D panda fixed-base manipulator with space-time constraints.}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/spacetime/well.png}
\caption{Subtask of well assembly.}
\end{subfigure}
\begin{subfigure}[t]{\width}
\centering
\includegraphics[width=\linewidth]{images/experiments/spacetime/pavillion.png}
\caption{Subtask of pavillion assembly.}
\end{subfigure}
\caption{Spacetime Experiments \label{fig:experiments:spacetime}.}
\end{figure*}

==> images/list_of_algorithms.tex <==

\newcolumntype{V}{>{\centering\arraybackslash}m{.003\linewidth}}
\newcolumntype{Z}{>{\raggedleft\arraybackslash}m{.12\linewidth}}
\newcolumntype{Y}{>{\centering\arraybackslash}m{.24\linewidth}}

\newcommand{\planner}[4]{%
#1 & #2 & #3 &
\xintFor ##1 in {#4} \do {
\xintifForFirst{}{&} 
\ifnum##1=1
%x
\fi
}
}

\begin{table*}[t]
    \centering
    \begin{tabularx}{\linewidth}{|Z|X|Y|V|V|V|V|V|V|}
    \hline
         \multicolumn{2}{|c|}{Motion Planning Algorithm} &
           Origin Paper &
         \multicolumn{6}{c|}{Properties}\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\multicolumn{9}{|c|}{Classical Motion Planner}\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Probabilistically complete, manifold support, asympt optimal, proj support
\planner{PRM}{Probabilistic Roadmap Planner}{\citep{Kavraki1996}}{1,1,0,0,0,1}\\
\planner{RRT}{Rapidly-exploring random tree}{\citep{Lavalle1998}}{1,1,0,0,0,1}\\
\planner{RRTConnect}{Bidirectional RRT}{\citep{Kuffner2000}}{1,1,0,0,0,1}\\
\planner{EST}{Expansive spaces planner}{\citep{Hsu1999}}{1,1,0,0,0,1}\\
\planner{BiEST}{Bidirectional EST}{\citep{Hsu1999}}{1,1,0,0,0,1}\\
\planner{LazyRRT}{Lazy edge evaluation RRT}{\citep{Kuffner2000}}{1,1,0,0,0,1}\\
\planner{TRRT}{Transition-based RRT}{\citep{Jaillet2010}}{1,1,0,0,0,1}\\
\planner{BiTRRT}{Bidirectional TRRT}{\citep{Jaillet2010}}{1,1,0,0,0,1}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\hline\multicolumn{9}{|c|}{Asymptotically Optimal Motion Planner}\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\planner{RRT*}{Optimal version of RRT}{\citep{Karaman2011}}{1,1,1,0,0,1}\\
\planner{PRM*}{Optimal version of PRM}{\citep{Karaman2011}}{1,1,1,0,0,1}\\
\planner{LazyPRM*}{Optimal version of LazyPRM}{\citep{Karaman2011}}{1,1,1,0,0,1}\\
\planner{RRT\#}{RRT sharp}{\citep{Arslan2013}}{1,1,1,0,0,1}\\
\planner{InformedRRT*}{Informed search RRT*}{\citep{Gammell2014}}{1,0,1,0,0,1}\\
\planner{SPARS}{Sparse roadmap spanners}{\citep{dobson_2014}}{1,1,1,0,1,1}\\
\planner{SPARS2}{SPARS w/o dense graph}{\citep{dobson_2014}}{1,1,1,0,1,1}\\
\planner{FMT}{Fast marching tree}{\citep{Janson2015}}{1,1,1,0,0,1}\\
\planner{BFMT}{Bidirectional FMT}{\citep{Janson2015}}{1,1,1,0,0,1}\\
\planner{LBTRRT}{Lower-bound tree RRT}{\citep{Salzman2016}}{1,1,1,0,0,1}\\
\planner{RRTX}{RRT /w pseudo-optimal tree}{\citep{Otte2016}}{1,1,1,0,0,1}\\
\planner{SORRT*}{Sorted InformedRRT*}{\citep{Li2016}}{1,0,1,0,0,1}\\
\planner{SST}{Stable sparse RRT}{\citep{Li2016}}{1,1,1,0,0,1}\\
\planner{BIT*}{Batch informed trees}{\citep{Gammell2020}}{1,0,1,0,0,1}\\
\planner{ABIT*}{Advanced BIT*}{\citep{Strub2020Advanced}}{1,0,1,0,0,1}\\
\planner{AIT*}{Adaptive BIT*}{\citep{Strub2020Adaptively}}{1,0,1,0,0,1}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\hline \multicolumn{9}{|c|}{Projection-Based Motion Planner}\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\planner{ProjEST}{Projection EST}{\citep{Hsu1999}}{1,1,0,1,0,1}\\
\planner{SBL}{Single-query bidirectional lazy PRM}{\citep{Sanchez2003}}{1,1,0,1,0,1}\\
\planner{PDST}{Path-Directed Subdivision Tree}{\citep{Ladd2004}}{1,1,0,1,0,1}\\
\planner{KPIECE}{\makecell[t]{Kinodynamic Motion Planning \\by Interior-Exterior Cell Exploration}}{\citep{Sucan2009}}{1,1,0,1,0,1}\\
\planner{BKPIECE}{Bidirectional KPIECE}{\citep{Sucan2009}}{1,1,0,1,0,1}\\
\planner{LBKPIECE}{Lazy BKPIECE}{\citep{Sucan2009}}{1,1,0,1,0,1}\\
\planner{STRIDE}{\makecell[t]{Search Tree with Resolution \\Independent Density Estimation}}{\citep{Gipson2013}}{1,1,0,1,0,1}\\
\planner{QMP/QMP*}{Quotient-space roadmap planner}{\citep{Orthey2018}}{1,1,1,1,0,1}\\
\planner{QRRT/QRRT*}{Rapidly-exploring random quotient space trees}{\citep{Orthey2019}}{1,1,1,1,0,1}\\
\planner{HBFMT*}{Hierarchical BFMT}{\citep{Reid2019}}{1,1,1,1,0,0}\\
%\planner{QRRT*}{Optimal version of QRRT}{\citep{Orthey2020IJRR}}{1,1,1,1,0,1}\\
%\planner{QMP*}{Optimal version of QMP}{\citep{Orthey2020IJRR}}{1,1,1,1,0,1}\\
\planner{XXL}{}{\citep{Luna2020}}{1,1,0,1,0,1}\\
\planner{SMLR}{Sparse Multilevel Roadmaps}{\citep{Orthey2021ICRA}}{1,1,1,1,1,1}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline 
\multicolumn{3}{l|}{}  &&&&&&\\
\cline{1-3}
\multicolumn{4}{|l|}{Probabilistically Complete} &&&&&\\
\cline{1-4}
\multicolumn{5}{|l|}{Supports Arbitrary Manifolds} &&&&\\
\cline{1-5}
\multicolumn{6}{|l|}{Asymptotically (near-)Optimal}&&&\\
\cline{1-6}
\multicolumn{7}{|l|}{Supports Projections}&&\\
\cline{1-7}        
\multicolumn{8}{|l|}{Asymptotic Sparsity}&\\
\cline{1-8}   
\multicolumn{9}{|l|}{Open source implementation in OMPL}\\
\cline{1-9}   
        
        \end{tabularx}
    \caption{List of motion planning algorithms used in experimental section. Properties of the algorithms are: Supporting fiber bundles (FB), being probabilistically complete (PC) and being asymptotically (near-)optimal (AnO).
    \label{tab:list_of_algorithms}}
\end{table*}

%\begin{table*}[t]
%    \centering
%    \begin{tabular}{|c|c|c|c|c|c|c|}
%    \hline
%         \multicolumn{2}{|c|}{Motion Planning Algorithm} &
%           Origin Paper &
%         FB &
%        PC & AnO & S\\
%        \hline
%        QRRT & \makecell[t]{Rapidly-exploring\\random quotient space trees} & \citep{orthey_2019} &x & x& &\\
%        QMP & Quotient-space roadmap planner & \citep{orthey_2018} &x & x&  &\\
%        QRRT* & Optimal version of QRRT & \textbf{this paper} &x & x& x &\\
%        QMP* & Optimal version of QMP & \textbf{this paper} &x & x& x &\\
%%        SPQR & Sparse Quotient-space roadmap & \textbf{this paper} &x & x& x & x\\
%        \hline
%        PRM & Probabilistic Roadmap Planner & \citep{kavraki_1996} & & x&  &\\
%        PRM* & Optimal version of PRM & \citep{karaman_2011} & & x &  &\\
%        LazyPRM* & Optimal version of LazyPRM & \citep{karaman_2011} & & x &  &\\
%        SPARS & Sparse roadmap spanners & \citep{dobson_2014} & & x & x  & x\\
%        SPARS2 & SPARS w/o dense graph & \citep{dobson_2014} & & x & x  & x\\
%        RRT & Rapidly-exploring random tree & \citep{lavalle_1998} & & x&  &\\
%        RRTConnect & Bidirectional RRT & \citep{kuffner_2000} & & x&  &\\
%        RRT* & Optimal version of RRT & \citep{karaman_2011} & & x &  &\\
%        LazyRRT & Lazy edge evaluation RRT & \citep{kuffner_2000} & & x & &\\
%        TRRT & Transition-based RRT & \citep{jaillet_2010} & & x & &\\
%        BiTRRT & Bidirectional TRRT & \citep{jaillet_2010} & & x & &\\
%        LBTRRT & Lower-bound tree RRT & \citep{salzman_2016} & & x &x &\\
%        RRTX & RRT /w pseudo-optimal tree & \citep{otte_2016} & & x & x &\\
%        RRT\# & RRT sharp & \citep{arslan_2013} &  & x &x &\\
%        InformedRRT* & Informed search RRT* & \citep{gammell_2014} & & x &x &\\
%        SORRT* & Sorted InformedRRT* & \citep{gammell_2014} & & x &x &\\
%        SBL & Single-query bidirectional lazy PRM & \citep{sanchez_2003} & & x & &\\
%        SST & Stable sparse RRT & \citep{li_2016} & & x &x &\\
%        STRIDE & \makecell[t]{Search Tree with Resolution \\Independent Density Estimation} & \citep{gipson_2013} & & x & &\\
%        FMT & Fast marching tree & \citep{janson_2015} & & x &x &\\
%        BFMT & Bidirectional FMT & \citep{janson_2015} & & x &x &\\
%        BIT* & Batch informed trees& \citep{gammell_2020} & & x &x &\\
%        ABIT* & Advanced BIT*& \citep{strub_2020} & & x &x &\\
%        EST & Expansive spaces planner& \citep{hsu_1999} & & x & &\\
%        BiEST & Bidirectional EST& \citep{hsu_1999} & & x & &\\
%        ProjEST & Projection EST& \citep{hsu_1999} & & x & &\\
%        KPIECE & \makecell[t]{Kinodynamic Motion Planning \\by Interior-Exterior Cell Exploration}& \citep{sucan_2009} & & x & &\\
%        BKPIECE & Bidirectional KPIECE& \citep{sucan_2009} & & x & &\\
%        LBKPIECE & Lazy BKPIECE& \citep{sucan_2009} & & x & &\\
%        PDST & Path-Directed Subdivision Tree& \citep{ladd_2004} & & x & &\\
%        \hline
%    \end{tabular}
%    \caption{List of motion planning algorithms used in experimental section. Properties are Fiber bundle enabled (FB), probabilistically complete (PC), asymptotically (near-)optimal (AnO) and sparse (S).}
%    \label{tab:list_of_algorithms}
%\end{table*}


==> images/list_of_planner_on_experiments.tex <==
\def\markYes{\color{red}{\checkmark}}
\def\markNo{{}}
\def\markUndef{\color{red}{E}}

\newcolumntype{P}{>{\centering\arraybackslash}m{.1\linewidth}}
\newcolumntype{Z}{>{\raggedleft\arraybackslash}m{.01\linewidth}}
\newcolumntype{+}{!{\vrule width 1.2pt}}
\begin{table*}[t]
\centering
\renewcommand\theadfont{\bfseries}
\footnotesize\centering
\renewcommand{\arraystretch}{1.2}
\setlength\tabcolsep{3pt}

\newcounter{plannerid}
\setcounter{plannerid}{1}
\newcommand{\addPlanner}[2]{%
\arabic{plannerid} & #1 & 
    \xintFor ##1 in {#2} \do {
        \xintifForFirst{}{&} 
        \ifnum##1=1
            \markYes
        \else
            \ifnum##1=-1
                \markUndef
            \else
                \markNo
            \fi
        \fi
    }
\stepcounter{plannerid}
}

\newcommand\Tstrut{\rule{0pt}{2ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-1ex]{0pt}{0pt}}   % = `bottom' strut
\newcommand{\addTopic}[1]{%
    \hline
    \multicolumn{}{|c|}{#1}\Tstrut\Bstrut\\
    \hline
}



\begin{tabularx}{\linewidth}{|ZX+|P|P|P|}\hline

\multicolumn{2}{|>{\centering}p{2.5cm}+}{Motion Planner}
 % Manifolds
 & Table of Relative Improvement
 & Table of Absolute Runtime
 & Optimality Graphs
 \\ \hline
\addPlanner{RRT}{1,1,0}\\
\addPlanner{RRTConnect}{1,1,0}\\
\addPlanner{RRT*}{1,1,1}\\
\addPlanner{RRTXstatic}{1,1,0}\\
\addPlanner{LazyRRT}{0,0,0}\\
\addPlanner{TRRT}{1,1,0}\\
\addPlanner{BiTRRT}{1,1,0}\\
\addPlanner{LBTRRT}{1,1,1}\\
\addPlanner{FMT}{1,1,1}\\
\addPlanner{BFMT}{1,1,1}\\
\addPlanner{RLRT}{1,1,0}\\
\addPlanner{BiRLRT}{1,1,0}\\
\addPlanner{PRM}{1,1,0}\\
\addPlanner{PRM*}{1,1,1}\\
\hline
\addPlanner{LazyPRM}{0,0,0}\\
\addPlanner{LazyPRM*}{0,0,0}\\
\hline
\addPlanner{SPARS}{1,1,1}\\
\addPlanner{SPARStwo}{1,1,1}\\
\addPlanner{SST}{1,1,1}\\
\addPlanner{EST}{1,1,0}\\
\addPlanner{BiEST}{1,1,0}\\
\hline
\addPlanner{QRRT}{0,0,0}\\
\addPlanner{QRRT*}{0,0,0}\\
\addPlanner{QMP}{0,0,0}\\
\addPlanner{QMP*}{0,0,0}\\
\addPlanner{SMLR}{0,0,0}\\
\addPlanner{CForest}{0,0,0}\\
\addPlanner{SORRT*}{0,0,0}\\
\hline
\addPlanner{InformedRRT*}{1,1,1}\\
\addPlanner{kBIT*}{1,1,1}\\
\addPlanner{kABIT*}{0,0,0}\\
\addPlanner{AIT*}{1,1,1}\\
\addPlanner{ProjEST}{0,0,0}\\
\addPlanner{PDST}{1,1,0}\\
\addPlanner{STRIDE}{1,1,0}\\
\addPlanner{KPIECE1}{1,1,0}\\
\addPlanner{BKPIECE1}{1,1,0}\\
\addPlanner{LBKPIECE1}{0,0,0}\\
\addPlanner{SBL}{1,1,0}\\

\hline
\end{tabularx}
\caption{Exclude: Lazy, Projections. Include: Bidirectional.}
\end{table*}


==> todo.tex <==
[ ] Make all experiments available online and clean them up
[ ] Write a small section for each experiment to say which algorithms performed best
[ ] Constantinos: Can you fix he hyperparameter selection section (7.1) ?
[ ] Constantinos: Can you add some references for constraint-based planning (4.4.4) ?



\section{NOTE (From IEEE)} 

A good survey paper must be more than an organized list of references. It must provide an authoritative and useful perspective and organization of the history and the state of the art of the field. It should include important references but leave out those that are minor or derivative contributions. It should not be biased toward the authors' own work. It should organize the material according to themes as appropriate (for example, applications or principles or technologies employed), and it should provide fair comparisons or critiques where appropriate. The authors should be acknowledged experts in the field. In short, a good survey paper should provide a perspective and distillation of the field that is a significant contribution in itself.

